Enhanced 3D Urban Scene Reconstruction and Point Cloud Densification using Gaussian Splatting and Google Earth Imagery

3D urban scene reconstruction and modelling is a crucial research area in remote sensing with numerous applications in academia, commerce, industry, and administration. Recent advancements in view synthesis models have facilitated photorealistic 3D reconstruction solely from 2D images. Leveraging Google Earth imagery, we construct a 3D Gaussian Splatting model of the Waterloo region centered on the University of Waterloo and are able to achieve view-synthesis results far exceeding previous 3D view-synthesis results based on neural radiance fields which we demonstrate in our benchmark. Additionally, we retrieved the 3D geometry of the scene using the 3D point cloud extracted from the 3D Gaussian Splatting model which we benchmarked against our Multi- View-Stereo dense reconstruction of the scene, thereby reconstructing both the 3D geometry and photorealistic lighting of the large-scale urban scene through 3D Gaussian Splatting

==> 00_abstract.tex <==
\begin{abstract}

3D urban scene reconstruction and modelling is a crucial research area. From a technical perspective, it is an interdisciplinary research area spanning across computer vision, computer graphics and photogrammetry. Its applications span across multiple disciplines including autonomous navigation with 3D scene understanding, remote sensing/photogrammetry for the creation of 3D maps from aerial/drone/satellite images, geographic information systems with urban digital twins, augmented and virtual reality with photorealistic scene reconstructions. Using Google Earth imagery, we create a 3D Gaussian Splatting model of the Waterloo region centered on the University of Waterloo, and are able to achieve view-synthesis results far exceeding previous 3D view-synthesis results based on neural radiance fields which we demonstrate in our benchmark. We also retrieve the 3D geometry of the scene using the 3D point cloud extracted from the 3D Gaussian Splatting model, thereby reconstructing both the 3D geometry and photorealistic lighting of the large-scale urban scene.
\end{abstract}

==> figs/Figuregrid3_halfsize.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view000.png}
    \end{subfigure}   
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view001.png}
    \end{subfigure}~
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view002.png}
    \end{subfigure}    
    
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view100.png}
    \end{subfigure}   
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view101.png}
    \end{subfigure}~
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view102.png}
    \end{subfigure}    

    \centering
\begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view200.png}
    \end{subfigure}   
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view201.png}
    \end{subfigure}~
    \begin{subfigure}[b]{0.15\textwidth}
\includegraphics[width = 1\textwidth, trim={15cm 7cm 15cm 3cm},clip]{figs/view202.png}
    \end{subfigure}    

   
\caption{3DGS point cloud densification visualization. Left: Fused dense and normal maps as ground truth (colored) point cloud. Middle: initial point cloud. Right: 3DGS densified point cloud.} \label{img:pc_compare}
\end{figure}
